Assessing Data Support for the Simplifying Assumption in Bivariate Conditional Copulas

The paper considers the problem of establishing data support for the simplifying assumption (SA) in a bivariate conditional copula model. It is known that SA greatly simplifies the inference for a conditional copula model, but standard tools and methods for testing SA tend to not provide reliable results. After splitting the observed data into training and test sets, the method proposed will use a flexible training data Bayesian fit to define tests based on randomization and standard asymptotic theory. Theoretical justification for the method is provided and its performance is studied using simulated data. The paper also discusses implementations in alternative models of interest, e.g. Gaussian, Logistic and Quantile regressions.

==> referenc.tex <==
\begin{thebibliography}{10}

\bibitem{agn}
E.F. Acar, C~Genest, and Johanna Ne\v{s}lehov\'a.
\newblock Beyond simplified pair-copula constructions.
\newblock {\em Journal of Multivariate Analysis}, 110:74--90, 2012.

\bibitem{acar2011dependence}
Elif~F Acar, Radu~V Craiu, and Fang Yao.
\newblock Dependence calibration in conditional copulas: A nonparametric
  approach.
\newblock {\em Biometrics}, 67(2):445--453, 2011.

\bibitem{acar2013statistical}
Elif~F Acar, Radu~V Craiu, Fang Yao, et~al.
\newblock Statistical testing of covariate effects in conditional copula
  models.
\newblock {\em Electronic Journal of Statistics}, 7:2822--2850, 2013.

\bibitem{gam-cc}
V.~Chavez-Demoulin and T.~Vatter.
\newblock Generalized additive models for conditional copulas.
\newblock {\em J. Multivariate Anal.}, 141:147--167, 2015.

\bibitem{choi2011gaussian}
Taeryon Choi, Jian~Q Shi, and Bo~Wang.
\newblock A {Gaussian} process regression approach to a single-index model.
\newblock {\em Journal of Nonparametric Statistics}, 23(1):21--36, 2011.

\bibitem{cra-sabeti}
Radu~V. Craiu and A.~Sabeti.
\newblock In mixed company: {B}ayesian inference for bivariate conditional
  copula models with discrete and continuous outcomes.
\newblock {\em J. Multivariate Anal.}, 110:106--120, 2012.

\bibitem{craiu2012mixed}
Radu~V. Craiu and Avideh Sabeti.
\newblock In mixed company: Bayesian inference for bivariate conditional copula
  models with discrete and continuous outcomes.
\newblock {\em Journal of Multivariate Analysis}, 110:106--120, 2012.

\bibitem{czado2010pair}
Claudia Czado.
\newblock Pair-copula constructions of multivariate copulas.
\newblock {\em Copula theory and its applications}, pages 93--109, 2010.

\bibitem{de2007modeling}
Jan De~Kort.
\newblock Modeling tail dependence using copulas-literature review.
\newblock {\em Faculty of Electrical Engineering, Mathematics and Computer
  Science (EEMCS), Delf University of Technology}, 2007.

\bibitem{derumigny2016tests}
Alexis Derumigny and Jean-David Fermanian.
\newblock About tests of the ``simplifying'' assumption for conditional
  copulas.
\newblock {\em Dependence Modeling}, 5(1):154--197, 2017.

\bibitem{embrechts2001modelling}
Paul Embrechts, Filip Lindskog, and Alexander McNeil.
\newblock Modelling dependence with copulas.
\newblock {\em Rapport technique, D{\'e}partement de math{\'e}matiques,
  Institut F{\'e}d{\'e}ral de Technologie de Zurich, Zurich}, 2001.

\bibitem{geisser1979predictive}
Seymour Geisser and William~F Eddy.
\newblock A predictive approach to model selection.
\newblock {\em Journal of the American Statistical Association},
  74(365):153--160, 1979.

\bibitem{genest1995semiparametric}
Christian Genest, Kilani Ghoudi, and L-P Rivest.
\newblock A semiparametric estimation procedure of dependence parameters in
  multivariate families of distributions.
\newblock {\em Biometrika}, 82(3):543--552, 1995.

\bibitem{gijbels2015estimation}
Ir{\`e}ne Gijbels, Marek Omelka, and No{\"e}l Veraverbeke.
\newblock Estimation of a copula when a covariate affects only marginal
  distributions.
\newblock {\em Scandinavian Journal of Statistics}, 42(4):1109--1126, 2015.

\bibitem{hanson}
T.~Hanson, A.~Branscum, and W.~Johnson.
\newblock Predictive comparison of joint longitudinal-survival modelling: a
  case study illustrating competing approaches.
\newblock {\em Lifetime Data Analysis}, 17:2--28, 2011.

\bibitem{hernandez2013gaussian}
Jos{\'e}~Miguel Hern{\'a}ndez-Lobato, James~R Lloyd, and Daniel
  Hern{\'a}ndez-Lobato.
\newblock Gaussian process conditional copulas with applications to financial
  time series.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1736--1744, 2013.

\bibitem{hu2013bayesian}
Yuao Hu, Robert~B Gramacy, and Heng Lian.
\newblock Bayesian quantile regression for single-index models.
\newblock {\em Statistics and Computing}, 23(4):437--454, 2013.

\bibitem{lamb-van}
Philippe Lambert and F~Vandenhende.
\newblock A copula-based model for multivariate non-normal longitudinal data:
  analysis of a dose titration safety study on a new antidepressant.
\newblock {\em Statist. Medicine}, 21:3197--3217, 2002.

\bibitem{lehmann2006testing}
Erich~L Lehmann and Joseph~P Romano.
\newblock {\em Testing statistical hypotheses}.
\newblock Springer Science \& Business Media, 2006.

\bibitem{levi2018bayesian}
Evgeny Levi and Radu~V Craiu.
\newblock Bayesian inference for conditional copulas using gaussian process
  single index models.
\newblock {\em Computational Statistics \& Data Analysis}, 122:115--134, 2018.

\bibitem{naish2007generalized}
Andrew Naish-Guzman and Sean Holden.
\newblock The generalized {FITC} approximation.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  1057--1064, 2007.

\bibitem{patton2006modelling}
Andrew~J Patton.
\newblock Modelling asymmetric exchange rate dependence*.
\newblock {\em International economic review}, 47(2):527--556, 2006.

\bibitem{quinonero2005unifying}
Joaquin Qui{\~n}onero-Candela and Carl~Edward Rasmussen.
\newblock A unifying view of sparse approximate gaussian process regression.
\newblock {\em The Journal of Machine Learning Research}, 6:1939--1959, 2005.

\bibitem{rasmussen2006gaussian}
Carl~Edward Rasmussen.
\newblock Gaussian processes for machine learning.
\newblock 2006.

\bibitem{sabeti2014additive}
Avideh Sabeti, Mian Wei, and Radu~V Craiu.
\newblock Additive models for conditional copulas.
\newblock {\em Stat}, 3(1):300--312, 2014.

\bibitem{Sklar:1959}
A.~Sklar.
\newblock Fonctions de r\'epartition \`a {$n$} dimensions et leurs marges.
\newblock {\em Publications de l'Institut de Statistique de l'Universit\'e de
  Paris}, 8:229--231, 1959.

\bibitem{vehtari2017practical}
Aki Vehtari, Andrew Gelman, and Jonah Gabry.
\newblock Practical bayesian model evaluation using leave-one-out
  cross-validation and waic.
\newblock {\em Statistics and Computing}, 27(5):1413--1432, 2017.

\bibitem{vog}
N~Veraverbeke, M.~Omelka, and Irene Gijbels.
\newblock Estimation of a conditional copula and association measures.
\newblock {\em Scand. J. Statist.}, 38:766--780, 2011.

\bibitem{watanabe2010asymptotic}
Sumio Watanabe.
\newblock Asymptotic equivalence of {Bayes} cross validation and widely
  applicable information criterion in singular learning theory.
\newblock {\em The Journal of Machine Learning Research}, 11:3571--3594, 2010.

\bibitem{watanabe2013widely}
Sumio Watanabe.
\newblock A widely applicable bayesian information criterion.
\newblock {\em Journal of Machine Learning Research}, 14(Mar):867--897, 2013.

\end{thebibliography}

